Tree search algorithms for the Sequential Ordering Problem

We present a study of several generic tree search techniques applied to the Sequential Ordering Problem. This study enables us to propose a simple and competitive tree search algorithm. It consists of an iterative Beam Search algorithm that favors search over inference and integrates dynamic programming inspired cuts. It proves optimality on half of the SOPLIB instances and finds new best known solutions on 6 among 7 open instances of the benchmark in a small amount of time.

==> old.tex <==
On the 6 still open instances of the dataset, our method finds new best solutions. On constrained instances R.X.X.30 and R.X.X.60, our method is also able to prove optimality in almost the same time as finding the optimal solution. On less constrained instances (\emph{i.e.} R.X.X.1), local searches and polyhedral approaches perform best and are able to close the instances. If we wanted to improve our results on those instances, we can integrate a local search scheme into our Beam Search to turn it into a Recovering Beam Search \cite{della2004recovering}. \cite{jamal2017solving} used this method with success on the SOP on R.X.X.1 instances.

best known LB (resp. UB) indicates the best bound values found in the literature. Beam Search indicates the value of the best solution found by our algorithm in 600s. time to record, indicates the time to find the optimal solution if it is known or to find a better solution than the best known.


\begin{center}
    \begin{tabular}{|l|l|l|l|l|l|}
\hline
name & n & best known lb & best known ub   & ub 30s & time to record (s) \\
\hline
ESC07 & 7 & 2.125 & 2.125                  & 2.125   & 0.001 \\
ESC11 & 11 & 2.075 & 2.075                 & 2.075   & 0.017 \\
ESC12 & 14 &1.675 & 1.675                  & 1.675   & 0.005 \\
ESC25 & 27 & 1.681 & 1.681                 & 1.681   & 15.853 (no proof) \\
ESC47 & 49 & 1.288 & 1.288                 & 1.500   & - \\
ESC63 & 65 & 62 & 62                       & 65      & - \\
ESC78 & 80 & 18.230 & 18.230               & 20.305  & - \\
br17.10 & 18 & 55 & 55                     & 55      & 0.011 (no proof) \\
br17.12 & 18 & 55 & 55                     & 55      & 0.006 (no proof) \\
ft53.1 & 54 & 7.531 & 7.531                & 8.537   & - \\
ft53.2 & 54 & 8.026 & 8.026                & 8.324   & - \\
ft53.3 & 54 & 10.262 & 10.262              & 11.166  & - \\
ft53.4 & 54 & 14.425 & 14.425              & 14.427  & - \\
ft70.1 & 71 & 39.313 & 39.313              & 42.120  & - \\
\textbf{ft70.2} & 71 & 40.101 & 40.419     & 42.346  & - \\
ft70.3 & 71 & 42.535 & 42.535              & 45.281  & - \\
ft70.4 & 71 & 53.530 & 53.530              & 54.062  & - \\
\textbf{kro124p.1} & 101 & 38.762 & 39.420 & 44.505  & - \\
\textbf{kro124p.2} & 101 & 39.841 & 41.336 & 48.696  & - \\
\textbf{kro124p.3} & 101 & 43.904 & 49.499 & 55.736  & - \\
\textbf{kro124p.4} & 101 & 73.021 & 76.103 & 79.809  & - \\
p43.1 & 44 & 28.140 & 28.140               & 29.200  & - \\
p43.2 & 44 &  28.480 & 28.480              & 29.010  & - \\
p43.3 & 44 &  28.835 & 28.835              & 29.285  & - \\
p43.4 & 44 &  83.005 & 83.005              & 83.015  & - \\
prob42 & 42 & 243 & 243                    & 276     & - \\
\textbf{prob100} & 100 & 1.045 & 1.163     & 1.671   & - \\
rbg048a & 50 & 351 & 351                   & 378     & - \\
rbg050c & 52 & 467 & 467                   & 573     & - \\
rbg109a & 111 & 1.038 & 1.038              & 1.060   & - \\
rbg150a & 152 & 1.750 & 1.750              & 1.804   & - \\
rbg174a & 176 & 2.033 & 2.033              & 2.141   & - \\
rbg253a & 255 & 2.950 & 2.950              & 3.103   & - \\
rbg323a & 325 & 3.140 & 3.140              & 3.349   & - \\
rbg341a & 343 & 2.568 & 2.568              & 2.873   & - \\
rbg358a & 360 & 2.545 & 2.545              & 3.126   & - \\
\textbf{rbg378a} & 380 & 2.809 & 2.816     & 3.326   & - \\
ry48p.1 & 49 & 15.805 & 15.805             & 17.542  & - \\
\textbf{ry48p.2} & 49 & 16.074 & 16.666    & 17.319  & - \\
\textbf{ry48p.3} & 49 & 19.490 & 19.894    & 20.546  & - \\
ry48p.4 & 49 & 31.446 & 31.446             & 31.446  & 4.311 (no proof) \\
\hline
    \end{tabular}
\end{center}


\appendix

\onecolumn
\begin{table}
    \centering
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
inst	& DFS\;\;	& DFS+PE\;\;	& BS\;\;	& BS+PE\;\;	& LDS\;\;	& LDS+PE\;\; \\
\hline
R.200.100.1	& 283	& 283	& 189	& 189	& 180	& 192 \\
R.200.100.15	& 3.940	& 3.740	& 1.796	& 1.792	& 3.114	& 2.325 \\
R.200.100.30	& 5.908	& \textbf{4.216}	& 4.249	& \textbf{4.216}	& 5.764	& 4.216 \\
R.200.100.60	& 75.875	& \textbf{71.749}	& 71.749	& \textbf{71.749}	& 75.063	& 71.749 \\
R.200.1000.1	& 3.526	& 3.448	& 2.554	& 2.554	& 2.684	& 2.684 \\
R.200.1000.15	& 40.185	& 34.836	& 20.517	& \textbf{20.481}	& 34.360	& 25.189 \\
R.200.1000.30	& 56.422	& \textbf{41.196}	& 41.728	& \textbf{41.196}	& 54.712	& 41.196 \\
R.200.1000.60	& 78.924	& \textbf{71.556}	& 71.556	& \textbf{71.556}	& 77.761	& 71.556 \\
\hline
R.300.100.1	& 259	& 265	& 204	& 214	& 206	& 225 \\
R.300.100.15	& 5.824	& 5.355	& 3.201	& 3.152	& 5.677	& 4.081 \\
R.300.100.30	& 8.737	& \textbf{6.120}	& 6.200	& \textbf{6.120}	& 8.115	& 6.120 \\
R.300.100.60	& 10.835	& \textbf{9.726}	& 9.726	& \textbf{9.726}	& 10.299	& 9.726 \\
R.300.1000.1	& 3.551	& 3.551	& 2.888	& 3.080	& 3.012	& 3.012 \\
R.300.1000.15	& 55.759	& 51.089	& 29.481	& 29.006	& 52.480	& 43.597 \\
R.300.1000.30	& 87.067	& 55.254	& 54.533	& \textbf{54.147}	& 84.200	& 54.147 \\
R.300.1000.60	& 124.463	& \textbf{109.471}	& 109.471	& \textbf{109.471}	& 122.803	& 109.471 \\
\hline
R.400.100.1	& 295	& 295	& 175	& 191	& 203	& 203 \\
R.400.100.15	& 8.513	& 8.103	& 3.961	& 3.879	& 7.438	& 6.584 \\
R.400.100.30	& 12.070	& \textbf{8.165}	& 8.183	& \textbf{8.165}	& 12.172	& 8.165 \\
R.400.100.60	& 17.062	& \textbf{15.228}	& 15.228	& \textbf{15.228}	& 17.017	& 15.228 \\
R.400.1000.1	& 4.620	& 4.466	& 3.247	& 3.247	& 3.298	& 3.525 \\
R.400.1000.15	& 78.492	& 76.454	& 39.722	& 38.963	& 73.798	& 69.342 \\
R.400.1000.30	& 122.816	& \textbf{85.128}	& 85.720	& \textbf{85.128}	& 120.821	& 85.128 \\
R.400.1000.60	& 158.276	& \textbf{140.816}	& 140.816	& \textbf{140.816}	& 155.713	& 140.816 \\
\hline
R.500.100.1	& 272	& 272	& 202	& 267	& 232	& 232 \\
R.500.100.15	& 10.833	& 9.917	& 5.411	& 5.261	& 10.590	& 9.610 \\
R.500.100.30	& 13.811	& 10.999	& 9.778	& \textbf{9.665}	& 13.801	& 9.665 \\
R.500.100.60	& 20.466	& \textbf{18.240}	& 18.257	& \textbf{18.240}	& 20.634	& 18.240 \\
R.500.1000.1	& 4.746	& 4.703	& 3.541	& 4.079	& 3.717	& 3.717 \\
R.500.1000.15	& 108.135	& 103.985	& 50.624	& 49.366	& 96.562	& 94.625 \\
R.500.1000.30	& 153.536	& 114.544	& 99.492	& \textbf{98.987}	& 147.592	& 98.987 \\
R.500.1000.60	& 203.281	& \textbf{178.212}	& 178.355	& \textbf{178.212}	& 200.655	& 178.212 \\
\hline
R.600.100.1	& 306	& 306	& 289	& 289	& 230	& 246 \\
R.600.100.15	& 13.029	& 13.007	& 5.695	& 5.469	& 11.263	& 10.939 \\
R.600.100.30	& 18.532	& 13.899	& 12.475	& \textbf{12.465}	& 18.137	& 12.465 \\
R.600.100.60	& 26.195	& \textbf{23.293}	& 23.324	& \textbf{23.293}	& 26.170	& 23.293 \\
R.600.1000.1	& 4.814	& 4.814	& 3.853	& 4.030	& 4.074	& 4.074 \\
R.600.1000.15	& 117.517	& 115.295	& 55.748	& 54.994	& 109.149	& 108.164 \\
R.600.1000.30	& 186.137	& 145.672	& 128.761	& \textbf{126.798}	& 181.128	& 126.798 \\
R.600.1000.60	& 248.143	& \textbf{214.608}	& 214.608	& \textbf{214.608}	& 252.814	& 214.608 \\
\hline
R.700.100.1	& 281	& 281	& 186	& 186	& 245	& 258 \\
R.700.100.15	& 14.337	& 13.778	& 7.220	& 7.020	& 13.742	& 13.206 \\
R.700.100.30	& 22.235	& 19.655	& 14.632	& \textbf{14.510}	& 22.216	& 14.510 \\
R.700.100.60	& 26.887	& \textbf{24.102}	& 24.102	& \textbf{24.102}	& 26.773	& 24.102 \\
R.700.1000.1	& 4.763	& 4.629	& 4.042	& 4.403	& 3.955	& 4.028 \\
R.700.1000.15	& 145.032	& 141.544	& 65.775	& 64.777	& 137.567	& 121.189 \\
R.700.1000.30	& 205.051	& 158.613	& 136.073	& \textbf{134.474}	& 203.240	& 134.474 \\
R.700.1000.60	& 275.111	& \textbf{245.589}	& 245.752	& \textbf{245.589}	& 273.659	& 245.589 \\
\hline
\end{tabular}
    \caption{Results for the prefix bound}
    \label{tab:prefix_bound}
\end{table}


\begin{table}
    \centering
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
inst	& DFS\;\;	& DFS+PE\;\;	& BS\;\;	& BS+PE\;\;	& LDS\;\;	& LDS+PE\;\; \\
\hline
R.200.100.1	& 283	& 283	& 189	& 189	& 180	& 192 \\
R.200.100.15	& 3.940	& 3.740	& 1.796	& 1.792	& 3.114	& 2.325 \\
R.200.100.30	& 5.908	& \textbf{4.216}	& 4.249	& \textbf{4.216}	& 5.764	& 4.216 \\
R.200.100.60	& 75.875	& \textbf{71.749}	& 71.749	& \textbf{71.749}	& 75.063	& 71.749 \\
R.200.1000.1	& 3.526	& 3.448	& 2.554	& 2.554	& 2.684	& 2.684 \\
R.200.1000.15	& 40.185	& 34.982	& 20.517	& \textbf{20.481}	& 34.360	& 25.592 \\
R.200.1000.30	& 56.422	& \textbf{41.196}	& 41.728	& \textbf{41.196}	& 54.712	& 41.196 \\
R.200.1000.60	& 78.924	& \textbf{71.556}	& 71.556	& \textbf{71.556}	& 77.761	& 71.556 \\
\hline
R.300.100.1	& 259	& 265	& 204	& 214	& 206	& 225 \\
R.300.100.15	& 5.824	& 5.371	& 3.201	& 3.152	& 5.687	& 4.081 \\
R.300.100.30	& 8.737	& \textbf{6.120}	& 6.200	& \textbf{6.120}	& 8.115	& 6.120 \\
R.300.100.60	& 10.835	& \textbf{9.726}	& 9.726	& \textbf{9.726}	& 10.299	& 9.726 \\
R.300.1000.1	& 3.564	& 3.551	& 2.888	& 3.080	& 3.012	& 3.012 \\
R.300.1000.15	& 55.759	& 51.152	& 29.481	& 29.006	& 52.480	& 43.597 \\
R.300.1000.30	& 87.067	& 55.791	& 54.533	& \textbf{54.147}	& 84.200	& 54.147 \\
R.300.1000.60	& 124.463	& \textbf{109.471}	& 109.471	& \textbf{109.471}	& 122.803	& 109.471 \\
\hline
R.400.100.1	& 295	& 295	& 175	& 191	& 203	& 203 \\
R.400.100.15	& 8.513	& 8.103	& 3.961	& 3.879	& 7.438	& 6.584 \\
R.400.100.30	& 12.070	& \textbf{8.165}	& 8.183	& \textbf{8.165}	& 12.172	& 8.165 \\
R.400.100.60	& 17.062	& \textbf{15.228}	& 15.228	& \textbf{15.228}	& 17.017	& 15.228 \\
R.400.1000.1	& 4.620	& 4.466	& 3.247	& 3.247	& 3.482	& 3.525 \\
R.400.1000.15	& 78.533	& 76.463	& 39.722	& 38.963	& 73.798	& 69.342 \\
R.400.1000.30	& 122.816	& \textbf{85.128}	& 85.720	& \textbf{85.128}	& 120.821	& 85.128 \\
R.400.1000.60	& 158.276	& \textbf{140.816}	& 140.816	& \textbf{140.816}	& 155.713	& 140.816 \\
\hline
R.500.100.1	& 272	& 272	& 202	& 275	& 232	& 232 \\
R.500.100.15	& 10.833	& 9.944	& 5.411	& 5.261	& 10.590	& 9.610 \\
R.500.100.30	& 13.811	& 11.059	& 9.778	& \textbf{9.665}	& 13.801	& 9.665 \\
R.500.100.60	& 20.466	& \textbf{18.240}	& 18.257	& \textbf{18.240}	& 20.634	& 18.240 \\
R.500.1000.1	& 4.746	& 4.703	& 3.541	& 4.079	& 3.717	& 3.717 \\
R.500.1000.15	& 108.135	& 103.985	& 50.624	& 49.366	& 96.562	& 94.625 \\
R.500.1000.30	& 153.536	& 115.693	& 99.492	& \textbf{98.987}	& 147.592	& 98.987 \\
R.500.1000.60	& 203.281	& \textbf{178.212}	& 178.355	& \textbf{178.212}	& 200.655	& 178.212 \\
\hline
R.600.100.1	& 308	& 306	& 289	& 289	& 230	& 246 \\
R.600.100.15	& 13.029	& 13.007	& 5.695	& 5.469	& 11.308	& 10.939 \\
R.600.100.30	& 18.532	& 13.952	& 12.475	& \textbf{12.465}	& 18.137	& 12.465 \\
R.600.100.60	& 26.195	& \textbf{23.293}	& 23.324	& \textbf{23.293}	& 26.170	& 23.293 \\
R.600.1000.1	& 4.814	& 4.814	& 3.853	& 4.030	& 4.074	& 4.074 \\
R.600.1000.15	& 117.517	& 115.295	& 55.748	& 54.994	& 109.149	& 108.164 \\
R.600.1000.30	& 186.137	& 146.815	& 128.761	& \textbf{126.798}	& 181.128	& 126.798 \\
R.600.1000.60	& 248.236	& \textbf{214.608}	& 214.608	& \textbf{214.608}	& 252.814	& 214.608 \\
\hline
R.700.100.1	& 281	& 281	& 186	& 250	& 245	& 258 \\
R.700.100.15	& 14.337	& 13.778	& 7.220	& 7.020	& 13.742	& 13.206 \\
R.700.100.30	& 22.235	& 19.723	& 14.632	& \textbf{14.510}	& 22.216	& 14.510 \\
R.700.100.60	& 26.887	& \textbf{24.102}	& 24.102	& \textbf{24.102}	& 26.773	& 24.102 \\
R.700.1000.1	& 4.763	& 4.639	& 4.042	& 4.403	& 3.955	& 4.028 \\
R.700.1000.15	& 145.032	& 141.544	& 65.775	& 64.777	& 137.567	& 121.189 \\
R.700.1000.30	& 205.051	& 159.040	& 136.073	& \textbf{134.474}	& 203.240	& 134.474 \\
R.700.1000.60	& 275.177	& \textbf{245.589}	& 245.752	& \textbf{245.589}	& 273.659	& 245.589 \\
\hline
\end{tabular}
    \caption{Results for the ingoing/outgoing bound}
    \label{tab:io_bound}
\end{table}


\twocolumn
